A Finite-Automaton Based Stream Cipher As a Quasigroup Based Cipher

In this paper we show that a recently published finite automaton stream cipher can be considered as a quasigroup based stream cipher. Some additional properties of the discussed cipher are also given.

==> eptcsdata.tex <==
\providecommand{\firstpage}{81}
\providecommand{\publicationstatus}{H. Bordihn, G. Horv\'ath, G. Vaszil (Eds.): 12th International Workshop on\\Non-Classical Models of Automata and Applications (NCMA 2022)\\
EPTCS 367, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.367.6}{10.4204/EPTCS.367.6}}
\pdfoutput=1

